Adaptive Granularity in Tensors: A Quest for Interpretable Structure

Data collected at very frequent intervals is usually extremely sparse and has no structure that is exploitable by modern tensor decomposition algorithms. Thus the utility of such tensors is low, in terms of the amount of interpretable and exploitable structure that one can extract from them. In this paper, we introduce the problem of finding a tensor of adaptive aggregated granularity that can be decomposed to reveal meaningful latent concepts (structures) from datasets that, in their original form, are not amenable to tensor analysis. Such datasets fall under the broad category of sparse point processes that evolve over space and/or time. To the best of our knowledge, this is the first work that explores adaptive granularity aggregation in tensors. Furthermore, we formally define the problem and discuss what different definitions of "good structure" can be in practice, and show that optimal solution is of prohibitive combinatorial complexity. Subsequently, we propose an efficient and effective greedy algorithm called IceBreaker, which follows a number of intuitive decision criteria that locally maximize the "goodness of structure", resulting in high-quality tensors. We evaluate our method on synthetic, semi-synthetic and real datasets. In all the cases, our proposed method constructs tensors that have very high structure quality.

==> dfn.tex <==

%%% DEFINITIONS COMMANDS
% \newcommand{\reminder}[1]{ {\bf *** #1 *** }  }
% \newcommand{\reminder}[1]{ {\bf *** #1 *** }  }
\newcommand{\reminder}[1]{{\textsf{\textcolor{red}  {[#1]}}}}
% \newcommand{\fromOld}[1] {{\textsf{\textcolor{green}{[#1]}}}}

%\newcommand{\comment}[1]{ {\tiny *** #1 *** }  }
\newcommand{\hide}[1]{}
% \newcommand{\sa}{\space}
\newcommand{\cleanup}{
    \renewcommand{\comment}{\hide}
    \renewcommand{\reminder}{\hide}
}
%% uncomment, to clean version
% \cleanup

\newcommand{\ben}{\begin{enumerate*}}
\newcommand{\een}{\end{enumerate*}}
% \newcommand{\bit}{\begin{itemize}}
% \newcommand{\eit}{\end{itemize}}
% \newcommand{\bit}{\begin{pitemize}}
% \newcommand{\eit}{\end{pitemize}}
\newcommand{\bit}{\begin{itemize*}}
\newcommand{\eit}{\end{itemize*}}
% \newcommand{\mypara}[1]{ \par \noindent \underline{ \em #1  } }
% \newcommand{\mypara}[1]{\par \noindent {\em #1}}
\newcommand{\mypara}[1]{\\ \par \noindent { #1}}


%\newtheorem{lemma}{Lemma}
% \newcommand{\comment}[1]{{\tiny #1 }}
\newcommand{\query}[1]{``{\em #1 }''}
% \newcommand{\reminder}[1]{{\bf *** #1 ***}}
% \renewcommand{\reminder}[1]{}
\newcommand{\fromOld}[1]{OLD STUFF {\tiny #1 }}

\newcommand{\QED}{ \hfill {\bf QED}}

\newcommand{\pegasus}{{\sc Pegasus}\xspace}

%\newcommand{\mytitle}{III: Small: Collaborative Research: Robust Mining of Coupled Tera-Scale Data: Where Hadoop Meets %Tensors.}

\newcommand{\mytitle}{BIGDATA:Mid-Scale:DA:Collaborative research:Big Tensor Mining: Theory, Scalable Algorithms and Applications.}

\newcommand{\ttensors}{XXXXXX}	% task numbers
\newcommand{\tfmri}{YYYYYY}
\newcommand{\tnet}{ZZZZZZ}
\newcommand{\tmethod}{2}	% task numbers
\newcommand{\tscale}{3}
\newcommand{\tapps}{1}
\newcommand{\tOtherApps}{2}

\newcommand{\hadoop}{\textsc{Hadoop}\xspace}
\newcommand{\htf}{\mbox{HTF}\xspace}


\newcommand{\nmethod}{Theory and methods}	% task numbers
\newcommand{\nmethodOne}{Multi-way Compressed Sensing}
\newcommand{\nmethodTwo}{Correlations as side information}
\newcommand{\nmethodThree}{Extensions for coupled multi-block data}


\newcommand{\nscale}{Scalability}
\newcommand{\bkw}{Brain-Knowledge-Web} 
\newcommand{\neurosemantics}{NeuroSemantics\xspace}
\newcommand{\napps}{Applications}
\newcommand{\nbkw}{Brain-Knowledge-Web Application}
\newcommand{\nOtherApps}{Recommendation Systems Application}
%\newcommand{\nOtherAppsTwo}{Time Evolving Call-Graph Application}
\newcommand{\nOtherAppsTwo}{Time Evolving Social Network Application}

\newcommand{\nscaleOne}{Optimized Tensor-Matrix-Vector Product Primitives}
\newcommand{\nscaleTwo}{Optimization Algorithms for Tensor Decomposition}
\newcommand{\nscaleThree}{Tensor Decomposition Algorithms}
\newcommand{\nscaleFour}{Software Development}


%\newcommand{\problem} {\noindent{\bf Problem Definition.}} 
\newcommand{\survey}   {\subsubsection{Literature survey}}
\newcommand{\current}  {\subsubsection{Current and Proposed Work}}

